Optimal Control of SOAs with Artificial Intelligence for Sub-Nanosecond Optical Switching

Novel approaches to switching ultra-fast semiconductor optical amplifiers using artificial intelligence algorithms (particle swarm optimisation, ant colony optimisation, and a genetic algorithm) are developed and applied both in simulation and experiment. Effective off-on switching (settling) times of 542 ps are demonstrated with just 4.8% overshoot, achieving an order of magnitude improvement over previous attempts described in the literature and standard dampening techniques from control theory.

==> SectionTemplate.tex <==
\section{Section Title} % Main section title









%-----------------------------------
%	MAIN SECTION
% INFO
% If this is the first section (i.e. the introduction), the very first letter is a 2 line initial drop letter followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.


% If this is not the first section (e.g. after introduction), don't need to use 2line initial drop letter(s). Can just write normally

% E.g. for introduction (first section): 
% \IEEEPARstart{T}{his} is how to write IEEE first section with 2 line initial drop letter

% For all other sections:
% This is how to write IEEE sections for all other sections

%-----------------------------------
\IEEEPARstart{T}{his} is how to write IEEE first section with 2 line initial drop letter \cite{WilliamMellette2018}














%-----------------------------------
%	SUB SECTION 1
%-----------------------------------

% \subsection{Subsection Heading Here}
% Subsection text here.











%-----------------------------------
%	SUB SUB SECTION 1
%-----------------------------------

% \subsubsection{Subsubsection Heading Here}
% Subsubsection text here.















































%-----------------------------------
%	EXTRA INFO
%-----------------------------------

% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.






















==> Sections/PreviousWork.tex <==
\section{Previous Work} % Main section title









%-----------------------------------
%	MAIN SECTION
% INFO
% If this is the first section (i.e. the introduction), the very first letter is a 2 line initial drop letter followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.


% If this is not the first section (e.g. after introduction), don't need to use 2line initial drop letter(s). Can just write normally

% E.g. for introduction (first section): 
% \IEEEPARstart{T}{his} is how to write IEEE first section with 2 line initial drop letter

% For all other sections:
% This is how to write IEEE sections for all other sections

%-----------------------------------
A previous attempt to optimise SOA output applied a `pre-impulse step injection current' (PISIC) driving signal to the SOA \cite{Gallep2002}. This PISIC signal pre-excited carriers in the SOA’s gain region, increasing the charge carrier density and the initial rate of stimulated emission to reduce the 10\% to 90\% rise time from 2 ns to 500 ps. However, this technique only considered rise time when evaluating SOA off-on switching times. A more accurate off-on time is given by the settling time, which is the time taken for the signal to settle within $\pm 5\%$ of the `on' steady state. Before settling, bits experience variable signal to noise ratio, which impacts the bit error rate (BER) makes the signal unusable until settled, therefore the switch is effectively `off' during this period.

A later paper looked at applying a `multi-impulse step injection current' (MISIC) driving signal to remedy the SOA oscillatory and overshoot behaviour \cite{Figueiredo2015}. As well as a pre-impulse, the MISIC signal included a series of subsequent impulses to balance the oscillations, reducing the rise time to 115 ps and the overshoot by 50\%. However, the method for generating an appropriate pulse format was trial-and-error. Since each SOA has slightly different properties and parasitic elements, the same MISIC format cannot be applied to different SOAs, therefore a different format must be generated through this inefficient manual process for each SOA, of which there will be thousands in a real DC. As such, MISIC is not scalable.  Critically, the MISIC technique did not consider the settling time, therefore the effective off-on switching time was still several ns.

The previous solutions discussed so far have had a design flow of first manually coming up with a heuristic for a simplified model of an SOA, followed by meticulous testing and tuning of the heuristic until good real-world performance is achieved. If some aspect of the problem is changed such as the SOA type used or the desired shape of the output signal, this process must be repeated. This paper presents a novel and scalable approach to optimising the SOA driving signal in an automated fashion with artificial intelligence (AI), requiring no prior knowledge of the SOA and being able to be generalised to any device without laborious manual configuration. Three algorithms were chosen on the basis that they had previously been applied to proportional-integral-derivative (PID) tuning in control theory \cite{7873803}: Particle swarm optimisation (PSO), ant colony optimisation (ACO), and a genetic algorithm (GA). All algorithms were shown to reduce the settling and rise times to the $O$(100ps) scale. The algorithms' hyperparameters were tuned in an SOA equivalent circuit (EC) simulation environment and their efficacy was demonstrated in an experimental setup. AI performance was compared to that of step, PISIC and MISIC driving signals as well as the popular raised cosine and PID control approaches to optimising oscillating and overshooting systems, all of which the AI algorithms outperformed.














%-----------------------------------
%	SUB SECTION 1
%-----------------------------------

% \subsection{Subsection Heading Here}
% Subsection text here.











%-----------------------------------
%	SUB SUB SECTION 1
%-----------------------------------

% \subsubsection{Subsubsection Heading Here}
% Subsubsection text here.















































%-----------------------------------
%	EXTRA INFO
%-----------------------------------

% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.





















